LEWIS (LayEr WIse Sparsity) -- A Training Free Guided Model Merging Approach

As specialized large language models (LLMs) become increasingly prevalent, model merging methods are being used to combine them to create a single multi-task model without requiring any additional data or training. However, these approaches fall short when the objective of merging is to increase the downstream model's performance on a particular task-specific benchmark. In this work, we propose LEWIS (Layer Wise Sparsity), a guided model-merging framework that uses activation-based layer importance to dynamically adjust layer-wise task-vector sparsity required for the merge process. LEWIS uses a calibration dataset to prioritize critical layers during the task-vector pruning process required for model merging. This approach guides existing merging methods by preserving essential layer-wise task-specific knowledge while ensuring the merged model performs the best at benchmarks resembling the calibration dataset. Our experiments demonstrate the effectiveness of LEWIS with performance improvements of code instruction-following and math-solving models created through model merging up to 4 percent and 11.3 percent, respectively, outperforming unguided data-less model merging approaches that use uniform-sparsity.

==> lewis.tex <==
\subsection{Preliminary Notations}
Given a Large Language Model (LLM) represented as a function \( f \), parameterized by \(\theta\), that maps a given prompt \( x \) to a generated output \( y \):
\[
y = f(x; \theta)
\]
where \(x \in \mathcal{X}\) is the input prompt from the input space \(\mathcal{X}\), and \(\theta \in \Theta\) represents the parameters of the model from the parameter space \(\Theta\). The parameters \(\theta\) encompass the weights and biases learned during the pre-training process. 


\subsubsection{Fine-Tuned Models on Multiple Tasks}
Fine-tuning a pre-trained LLM involves adapting the model's parameters to specialize in a specific task. Let the pre-trained model be parameterized by \(\theta_0\), and the fine-tuned model for a task \(T\) be parameterized by \(\theta_T\). The difference between these parameter sets, referred to as the \textit{task vector}, is defined as:
\[
\Delta \theta_T = \theta_T - \theta_0
\]
where \(\Delta \theta_T\) represents the adjustments made to the pre-trained model's parameters to optimize for task \(T\).

Now, consider a series of LLMs, denoted by \(\{\mathcal{M}_p\}_{p=1}^P\), where each model \(\mathcal{M}_p\) is fine-tuned on a distinct task \(p\). Each fine-tuned model can be expressed as:
\[
\mathcal{M}_p = f(x; \theta_p)
\]
where:
\[
\theta_p = \theta_0 + \Delta \theta_p
\]
Here:
\begin{itemize}
    \item \(\Delta \theta_p\): The task vector capturing the parameter adjustments for task \(p\).
    \item \(\theta_p\): The parameters of the fine-tuned model for task \(p\).
\end{itemize}


\subsubsection{Merging Fine-Tuned LLMs}
We can efficiently combine multiple fine-tuned models by treating the parameter changes as vectors in the parameter space. For example, when merging models fine-tuned for tasks \(T_1, T_2, \dots, T_n\), the merged model's parameters can be expressed as:
\[
\theta_{\text{merged}} = \theta_0 + \sum_{i=1}^n \alpha_i \cdot g(\Delta \theta_{T_i})
\]
where:
\begin{itemize}
    \item \(\theta_{\text{merged}}\) is the parameter set of the merged model.
    \item \(\alpha_i \in \mathbb{R}\) are scaling coefficients that control the contribution of each task vector \(\Delta \theta_{T_i}\).
    \item The pruning function \(g(\cdot)\) may be defined based on certain task vector redundancy criterions, more generally seen in TIES\cite{yadav2024ties}, DARE \cite{yu2024language} and inspired methods.   
    \item \(n\) is the number of tasks being merged.
\end{itemize}

\subsubsection{Calibration Dataset}
Let \(\mathcal{D} = \{x_i\}_{i=1}^N\) be a calibration dataset with \(N\) samples. This dataset is used to guide the merging process by providing representative data that allows us to optimize the performance of the merged model. By leveraging the calibration dataset \(\mathcal{D}\), the merged model can be tuned to perform optimally on tasks that resemble the characteristics of \(\mathcal{D}\).


% \subsection{Lewis: Model Merging using Layer Importance}

% To ensure an effective merging process, we determine the importance of each layer in the fine-tuned models by analyzing their activations using the calibration dataset. The steps for this process are as follows:

% \subsubsection*{Step 1: Pass Calibration Dataset Through Models}
% For each model \(\mathcal{M}_p\), pass the calibration dataset \(\mathcal{D} = \{x_i\}_{i=1}^N\) through the model to obtain activations. Let \(A_{(p, l)}(x_i)\) represent the activation at layer \(l\) for sample \(x_i\) in model \(\mathcal{M}_p\).

% \subsubsection*{Step 2: Compute Norms of Layers}
% Compute the norm of the activations for each layer \(l\) across the entire dataset \(\mathcal{D}\). The norm for layer \(l\) in model \(\mathcal{M}_p\) is calculated as:
% \[
% \text{Norm}_{(p, l)} = \frac{1}{N} \sum_{i=1}^N \|A_{(p, l)}(x_i)\|
% \]
% where \(\|\cdot\|\) represents an appropriate norm (e.g., \(L_2\)-norm).
% \subsubsection*{Step 3: Compare and Normalize Differences with Pre-Trained Model Activations}
% For each layer \(l\), the activation norms of the pre-trained model \(\mathcal{M}_{\text{pre-trained}}\) and the fine-tuned model \(\mathcal{M}_p\) are compared as follows:
% \begin{enumerate}
%     \item Compute the absolute difference between the activation norms of the pre-trained and fine-tuned models:
%     \[
%     \Delta A_{(p, l)} = \left| \text{Norm}_{(p, l)} - \text{Norm}_{\text{pre-trained}, l} \right|
%     \]
%     where \(\text{Norm}_{(p, l)}\) and \(\text{Norm}_{\text{pre-trained}, l}\) are the norms of activations at layer \(l\) for the fine-tuned and pre-trained models, respectively.

%     \item Normalize the differences across all layers in the model to ensure that the total importance sums to 1:
%     \[
%     \Delta A_{(p, l)} \leftarrow \frac{\Delta A_{(p, l)}}{\sum_{l} \Delta A_{(p, l)}}
%     \]
%     If the sum is zero, normalization is skipped to avoid division by zero.
%     \item Clip the normalized values to the range \([\gamma, \epsilon]\), where \(\gamma\) and \(\epsilon\) are empirically determined constants:
%     \[
%     \Delta A_{(p, l)} \leftarrow \text{clip}(\Delta A_{(p, l)}, \gamma, \epsilon)
%     \]
% \end{enumerate}



% \subsubsection*{Step 4: Use Differences to Determine Pruning Function}
% The activation differences \(\Delta A_{(p, l)}(x_i)\) across the calibration dataset are used directly to decide the pruning strategy. Layers that exhibit higher differences between the fine-tuned and pre-trained models are pruned less, while layers with smaller differences are pruned more. The pruning function \(g(l, p)\) for each layer \(l\) in model \(\mathcal{M}_p\) is defined as:
% \[
% g(l, p) \propto \Delta A_{(p, l)}(x_i)
% \]


% \subsubsection*{Step 5: Define Unique \(g\) Function for Each Layer}
% A unique pruning function \(g(l, p)\) is defined for each layer \(l\) across all models \(\mathcal{M}_p\), based on the task-specific differences:
% \[
% g(l, p) \propto \Delta A_{(p, l)}
% \]



\begin{algorithm}[h]
\caption{Lewis: Model Merging using Layer Importance}
\label{alg:lewis}
\begin{algorithmic}[1]
\Require 
\begin{itemize}
    \item Pre-trained model parameters: $\theta_0$
    \item Fine-tuned models: $\{\mathcal{M}_p\}_{p=1}^P$ with parameters $\{\theta_p\}_{p=1}^P$
    \item Calibration dataset: $\mathcal{D} = \{x_i\}_{i=1}^N$
    \item Pruning bounds: $[\gamma, \epsilon]$
\end{itemize}
\Ensure Merged model parameters: $\theta_{\mathrm{merged}}$

\Statex

\Procedure{LewisMerging}{$\theta_0, \{\theta_p\}, \mathcal{D}$}
    \State \textbf{Step 1: Pass Calibration Dataset Through Models}
    \For{$p = 1$ to $P$}
        \For{$x_i \in \mathcal{D}$}
            \State Obtain layer activations $A_{(p, l)}(x_i)$ for all layers $l$ of $\mathcal{M}_p$
        \EndFor
    \EndFor

    \State \textbf{Step 2: Compute Norms of Layers}
    \For{$p = 1$ to $P$}
        \For{each layer $l$}
            \State $\text{Norm}_{(p, l)} \gets \frac{1}{N} \sum_{i=1}^N \|A_{(p, l)}(x_i)\|$
        \EndFor
    \EndFor
    \State Similarly compute $\text{Norm}_{\mathrm{pre-trained}, l}$ for the pre-trained model.

    \State \textbf{Step 3: Compare and Normalize Differences with Pre-Trained Model Activations}
    \For{$p = 1$ to $P$}
        \For{each layer $l$}
            \State $\Delta A_{(p,l)} \gets \left|\text{Norm}_{(p, l)} - \text{Norm}_{\mathrm{pre-trained}, l}\right|$
        \EndFor
        \State $S \gets \sum_{l} \Delta A_{(p,l)}$
        \If{$S \neq 0$}
            \For{each layer $l$}
                \State $\Delta A_{(p,l)} \gets \frac{\Delta A_{(p,l)}}{S}$
                \State $\Delta A_{(p,l)} \gets \mathrm{clip}(\Delta A_{(p,l)}, \gamma, \epsilon)$
            \EndFor
        \EndIf
    \EndFor

    \State \textbf{Step 4: Use Differences to Determine Pruning Function}
    \For{$p = 1$ to $P$}
        \For{each layer $l$}
            \State Define pruning function $g(l, p) \propto \Delta A_{(p,l)}$
            \Comment{Higher $\Delta A_{(p,l)}$ = lower pruning rate}
        \EndFor
    \EndFor

    \State \textbf{Combine Models (Optional)}
    \State $\theta_{\mathrm{merged}} \gets \theta_0 + \sum_{p=1}^P \alpha_p \cdot g(\Delta \theta_p)$
    \Comment{Use any weighting or pruning as defined}
    
    \State \textbf{return} $\theta_{\mathrm{merged}}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


